Graded Hoare Logic and its Categorical Semantics

Deductive verification techniques based on program logics (i.e., the family of Floyd-Hoare logics) are a powerful approach for program reasoning. Recently, there has been a trend of increasing the expressive power of such logics by augmenting their rules with additional information to reason about program side-effects. For example, general program logics have been augmented with cost analyses, logics for probabilistic computations have been augmented with estimate measures, and logics for differential privacy with indistinguishability bounds. In this work, we unify these various approaches via the paradigm of grading, adapted from the world of functional calculi and semantics. We propose Graded Hoare Logic (GHL), a parameterisable framework for augmenting program logics with a preordered monoidal analysis. We develop a semantic framework for modelling GHL such that grading, logical assertions (pre- and post-conditions) and the underlying effectful semantics of an imperative language can be integrated together. Central to our framework is the notion of a graded category which we extend here, introducing graded Freyd categories which provide a semantics that can interpret many examples of augmented program logics from the literature. We leverage coherent fibrations to model the base assertion language, and thus the overall setting is also fibrational.

==> cut.tex <==

\begin{example}[Bounded reading via a graded comoandic semantics]
\label{exm:graded-comonad}
In the bounded reading example (Example~\ref{exm:cardinality}),
grades provides a count of the number of times each mutable program
variable is read throughout a program with \pmonoid{} of natural-number
vectors $(\mathbb{N}^N, \leq, 0_N, +)$ for $N$ program variables. We
can model this instance of GHL via a graded comonad akin to models
of exact usage analysis in functional `coeffect'
calculi~\cite{DBLP:conf/icfp/GaboardiKOBU16}. Let the base category
$(\CC, \otimes, I)$ be some symmetric monoidal category over which
we have a graded comonad, graded by the additive natural number monoid
\dnote{Oh no this doesn't work.. hm...}
with less-than-equal ordering $\leq$:
%
\begin{align*}
!_r A = A^r \qquad
\epsilon : !_1 A \rightarrow A =
\end{align*}
%
\dnote{WIP}
\end{example}

\begin{example}[Dataflow-Aware Reuse Bounds] % effe-notes
  \label{exm:dataflow}
  \dnote{OUT OF DATE NOW- Needs updating to $f$}
  A more interesting analysis is provided by a preordered monoid of
  square matrices containing natural numbers, which computes the
  data-flow paths of variables through the program.

  Let $\mathcal{M}$ be the set of $\mathbb{N}^{N \times N}$ of
  $N \times N$ matrices, with a preordered monoid structure via binary
  operation $\fatsemi$:
  %
  \begin{equation*}
    A \fatsemi B = (B \ast A) + A + B
  \end{equation*}
  %
  with the all-zeros matrix $\bar{0}_{N \times N}$ as the unit and
  preordering by pointwise $\leq$ on
  $\mathbb{N}$.\marginpar{\dnote{Sure about this preordering?}}  The
  analysis of expressions is defined in terms of the $\countVar$
  function in Example~\ref{exm:cardinality} where the analysis on an
  expression $\expr{v}{e}$ is defined:
%
  \begin{equation*}
    \expr{v_i}{e} = \transpose{J_i} \ast \countVar{e}
  \end{equation*}
%
  i.e., multiplication of the vector $\countVar{e}$ by the transpose
  of the single entry vector for variable $i$ (a column vector),
  yielding an $N \times N$ data flow matrix.

  For example, take the program $x := y + 2; z := x + y$ from the
  previous example. The three variables $x$, $y$ and $z$ are assigned
  their lexicographic order in the analysis.  The first assignment has
  the analysis:
%
  \setlength\arraycolsep{3pt}
  \begin{align*}
    \expr{x}{y + 2} =
    \transpose{J_x} \ast \countVar{y+2} =
    \begin{bmatrix} 1 \\ 0 \\ 0 \end{bmatrix}
    \ast
    \begin{bmatrix} 0 & 1 & 0 \end{bmatrix} =
                            \begin{bmatrix}
                              0 & 1 & 0 \\
                              0 & 0 & 0 \\
                              0 & 0 & 0
                            \end{bmatrix}
                            % Alt view
                            % \begin{array}{rccc}
                            %   \text{trg $\backslash$ src} & x & y &
     % z \\
     %x & \multicolumn{3}{c}{\multirow{3}{*}{$\begin{bmatrix}
     % %& x & y & z \\
     %   0 & 0 & 0 \\
     %   1 & 0 & 0 \\
     %   0 & 0 & 0
    %\end{bmatrix}$}} \\
    % y & \\
    % z &
    %\end{array}
\end{align*}
%
The resulting matrix can read as follows: the columns correspond to the
source of the dataflow and the rows the target, thus
in this case we see that $y$ (second variable) is used once to form
$x$ (first variable).
The second assignment has the analysis:
%
\begin{align*}
  \expr{z}{x + y} =
  \transpose{J_z} \ast \countVar{x+y} =
  \begin{bmatrix} 0 \\ 0 \\ 1 \end{bmatrix}
  \ast
  \begin{bmatrix} 1 & 0 & 1 \end{bmatrix} =
    \begin{bmatrix}
      0 & 0 & 0 \\
      0 & 0 & 0 \\
      1 & 1 & 0
    \end{bmatrix}
\end{align*}
%
Taken together using $\fatsemi$ from the sequential composition, the
full program then has the analysis:
%
\begin{align*}
 & \begin{bmatrix}
      0 & 1 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & 0
    \end{bmatrix}
\fatsemi
    \begin{bmatrix}
      0 & 0 & 0 \\
      0 & 0 & 0 \\
      1 & 1 & 0
    \end{bmatrix} \\
= \; &
  \begin{bmatrix}
      0 & 0 & 0 \\
      0 & 0 & 0 \\
      1 & 1 & 0
    \end{bmatrix}
\!\!\ast\!\!
    \begin{bmatrix}
      0 & 1 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & 0
    \end{bmatrix}
+
\begin{bmatrix}
      0 & 1 & 0 \\
      0 & 0 & 0 \\
      0 & 0 & 0
    \end{bmatrix}
+
    \begin{bmatrix}
      0 & 0 & 0 \\
      0 & 0 & 0 \\
      1 & 1 & 0
    \end{bmatrix}
%& =
%  \begin{bmatrix}
%      0 & 0 & 0 \\
%      0 & 0 & 0 \\
%      0 & 1 & 0
%    \end{bmatrix}
%+
%\begin{bmatrix}
%      0 & 1 & 0 \\
%      0 & 0 & 0 \\
%      0 & 0 & 0
%    \end{bmatrix}
%+
%    \begin{bmatrix}
%      0 & 0 & 0 \\
%      0 & 0 & 0 \\
%      1 & 1 & 0
%    \end{bmatrix} \\
\; =
\begin{bmatrix}
      0 & 1 & 0 \\
      0 & 0 & 0 \\
      1 & 2 & 0
    \end{bmatrix}
\end{align*}
%
Thus, $y$ flows once to $x$ and twice to $z$ and $x$ flows once to
$z$. The analysis of individual statements essentially gives an adjacency
matrix for the dataflow graph of the statement and $\fatsemi$ computes the two-hop paths
between the two dataflow graphs $(B \ast A)$ plus
the original adjacency/flows $A$ and $B$ for each statement.

\dnote{So far these examples are boring in the sense that they do not
  show an interaction between the proposition of the Hoare triples and
  the grades, which is the main interesting thing really.}
\end{example}

\begin{example}[Security Levels] % effe-notes

\end{example}

\subsection{Extended resource bounds}

Carbonneaux et al. present a quantitative verification approach for
amortized cost analysis via a Hoare logic augmented with multivariate
quantities associated to program
variables~\cite{DBLP:conf/pldi/Carbonneaux0S15}.  Their judgments are
of the form $\vdash \{\Gamma; Q\} S \{\Gamma'; Q'\}$ where $\Gamma$
and $\Gamma'$ are the usual pre- and post-conditions and $Q$ and $Q'$
are quantitative annotation functions mapping from indices
$i \in I = \{0\} \cup \{(x, y) \mid x, y \in \Var \wedge x \neq y\}$
to rational numbers. The meaning is that: if statement $S$ is executed
with starting state $\sigma$ for which assertions $\Gamma$ hold and at
least $Q @ \sigma$ resources are available before executing (where $@$
relates the annotation to the cost associated with state $\sigma$, our
notation). Then the evaluation succeeds with a state $\sigma'$ such
that $\Gamma'$ holds for this state and there are at least
$Q' @ \sigma'$ resources left. (Some additional accounting is included
in their judgments for loop breaks and function calls, but we elide
this here for simplicity). Thus their system has input and output
potentials function $Q$ and $Q'$.

Their approach can be mapped to our Graded Hoare Logic with a grading
monoid
$\mathcal{M} = (I \rightarrow \mathbb{Q}^+_0) \rightarrow (I
\rightarrow \mathbb{Q}^+_0)$ with the identity function as the unit
element and sequential composition as the binary operation, i.e.,
$(\mathcal{M}, \circ, \textit{id})$.  For example, the core rules of
function composition for Carbonneaux et al., shown on the left of
$\Longrightarrow$ are mapped into those on the right of
$\Longrightarrow$ in our system:
 %
\begin{align*}
  & \vdash \{\Gamma; Q\}\ \synSkip\ \{\Gamma; Q\} \;\; \\
  \Longrightarrow \;\; &
                         \vdash_{id_Q} \, \{\Gamma\}\ \synSkip\ \{\Gamma\}
  \\[2em]
  & \dfrac{\{\Gamma; Q\} S_1\ \{\Gamma', Q'\} \quad \{\Gamma'; Q'\}
    S_2\ \{\Gamma'', Q''\}}
    {\{\Gamma; Q\} S_1; S_2\ \{\Gamma'', Q''\}} \\
  \Longrightarrow \;\;  &
                          \dfrac{\tripleV{f}{\Gamma}{P_1}{\Gamma'}
                          \quad \tripleV{g}{\Gamma'}{P_2}{\Gamma''}}
                          {\tripleV{g \circ f}{\Gamma}{S_1; S_2}{\Gamma'}}
\end{align*}
 %
 %
\dnote{Say something about the functional representation being more
  perspicuous than their abstracted relational style?}  \dnote{Note,
  once we get the interesting rules we need to convert additions to
  pre-condition information (input) to subtractions on the post-
  (output)} \dnote{TODO: finish this section}


==> discussion.tex <==
\subsection{2-categorical categorisation}

A central concept in this paper is graded Freyd
categories. In this section we outline an alternative, abstract
definition of $M$-graded Freyd category using $2$-categorical
language.  In summary, a graded Freyd category is an equivalent
morphism in the category of actions of a cartesian category to
$M$-graded categories.  This conceptual formulation yields Definition
\ref{def:freydcoprod}.%of
%This formulation

For a \pmonoid{} $M$, the category of covariant presheaves $[M,\Set]$
has a monoidal structure by Day's convolution product. Then $M$-graded
categories are precisely $[M,\Set]$-enriched categories.  It is
therefore natural to define $M$-graded functors and $M$-graded natural
transformations as $[M,\Set]$-enriched functors and
$[M,\Set]$-enriched natural transformations. We write $\CATg M$ for
the 2-category of $M$-graded categories, $M$-graded functors and
$M$-graded natural transformations.  Of course $\CATg 1$ is isomorphic
to the category $\CAT$ of locally small categories.  There are two
2-functors: the underlying-category functor $U:\CATg M\arrow\CAT$ and
the constant-hom-presheaf functor $E:\CAT\arrow\CATg M$, which is
induced by the unique monoid homomorphism $M\arrow 1$. The 2-functor
$U$ also has a left 2-adjoint $L:\CAT\arrow\CATg M$.

We next introduce the concept of \emph{actions} of a cartesian monoidal
category $(\VV,1,\times)$ on an $M$-graded category $\CC$. It is
defined as a strong monoidal functor
$(\VV,1,\times) \arrow(\CATg M(\CC,\CC),Id,\circ)$. We form the
category $\Act\VV M$ of actions, where an object is a pair of an
$M$-graded category $\CC$ and an action
$(*):(\VV,1,\times)\arrow(\CATg M(\CC,\CC),\Id,\circ)$ on
it. Morphisms are $M$-graded functors satisfying equivariant
axioms. For example, every cartesian category $(\VV,1,\times)$
induces an action of $\VV$ on $L\VV$:
\begin{displaymath}
  L_{\VV,\VV}\circ (\times):
  (\VV,1,\times)\arrow
  (\CAT (\VV,\VV),\Id,\circ)\arrow
  (\CATg M(L\VV,L\VV),\Id,\circ)
\end{displaymath}
We then let $\mathcal L_\VV\teq (L\VV,L_{\VV,\VV}\circ (\times))\in\Act\VV M$.
We are ready to define $M$-graded Freyd category.
\begin{definition}
  An $M$-graded Freyd category consists of an action
  $\mathcal C\in\Act\VV M$ and an equivariant morphism
  $I:\mathcal L_\VV\arrow\mathcal C$ which is also identity-on-object.
\end{definition}
The unfolding of this definition is Definition \ref{def:freydcoprod}.




==> freyd.tex <==
% -*- mode: LaTeX; TeX-master: "main.tex"; -*-

\section{2-Categorical Formulation of Graded Categories\conf{50}}
\label{sec:2-cat}

In this section we develop an abstract theory of graded categories.
The goal is to give a concise formulation of graded Freyd categories
in Section \ref{...}. This gives an abstract characterization
of graded Freyd categories.

We first introduce
An \emph{$M$-graded functor} from an $M$-graded category $\CC$
to another one $\DD$ consists of the following data:
\begin{itemize}[leftmargin=1.5em]
\item A function $F:\Obj\CC\arrow\Obj\DD$.
\item A family $F_{I,J,m}:\CC(I,J)(m)\arrow\DD(FI,FJ)(m)$ of
  functions, satisfying
  \begin{displaymath}
    F_{I,I,1}(\id_I)=\id_{FI},\quad
    F_{I,K,m\cdot n}(f\circ g)=F_{n,J,K}(f)\circ F_{I,J,m}(g),\quad
    F_{I,J,n}(\up I J m n f)=\up{FI}{FJ}m n (F_{I,J,m}(f)).
  \end{displaymath}
\end{itemize}
An \emph{$M$-graded natural transformation} between $M$-graded
functors $F,G:\CC\arrow\DD$ is a family of morphisms
$\alpha_I:FI\arrow_1 GI$ in $\DD$ such that for any $f:I\arrow_m J$ in
$\CC$, we have $\alpha_J\circ Ff=Gf\circ\alpha_I$.  By $\CATg M$ we
mean the 2-category of $M$-grade categories, $M$-graded functors and
$M$-graded natural transformations between them.  $\CATg 1$ is
isomorphic to the 2-category of locally small categories, hence we
simply write it by $\CAT$.

The 2-category $\CAT_M$ has small 2-products. We here look at the
binary case. For $M$-graded categories $\CC,\DD$, we define
$\CC\times\DD$ by:
\begin{itemize}
\item $\Obj{\CC\times\DD}=\Obj\CC\times\Obj\DD$,
\item $(\CC\times\DD)((I,J),(I',J'))(m)=\CC(I,I')(m)\times\DD(J,J')(m)$.
\item The identity and composition are defined componentwisely.
\end{itemize}
We have obtained the 2-category $\Cat_M$ for each \pmonoid{}
 $M$.  For the systematic study of graded categories, it is also
convenient to understand how a monotone monoid homomorphism
$h:M\arrow N$ between partially ordered monoids $M,N$ induces a
2-functor $h^*:\Cat_N\arrow\Cat_M$.
\begin{itemize}
\item For a 0-cell $\CC\in\Cat_N$, we define the 0-cell
  $h^*\CC\in\Cat_M$ by
  \begin{align*}
    \Obj{h^*\CC}&\triangleq\Obj{\CC},&
    (h^*\CC)(I,J)(m)&\triangleq\CC(I,J)(h(m)),&
    \up I J m {m'}&\triangleq \up I J {h(m)} {h(m')}.%:(h^*\CC)(I,J)(m)\arrow(h^*\CC)(I,J)(m').
  \end{align*}
\item For a 1-cell $F:\CC\arrow\DD$ in $\Cat_N$, we define
  the 1-cell $h^*\alpha:h^*\CC\arrow h^*\DD$ by
  \begin{align*}
    (h^*F)(I)&\triangleq FI
    & (h^*F)_{I,J,m}(f)&\triangleq F_{I,J,h(m)}(f)
  \end{align*}
\item For a 2-cell $\alpha:F\arrow G$ in $\Cat_N$, we define the
  2-cell $h^*F:h^*F\arrow h^*G$ by $(h^*\alpha)_I\triangleq\alpha_I$.
\end{itemize}
It is routine to verify that this indeed determines a 2-functor
$h^*:\Cat_N\arrow\Cat_M$ strictly preserving small 2-products. Here we
look at two important instances of this 2-functor, involving the
one-point trivial monoid $1$.
\begin{enumerate}
\item The unique monoid homomorphism $e_M:1\arrow M$, specifying the
  unit $1$ of the monoid $M$, determines the 2-functor
  $e_M^*:\Cat_M\arrow\Cat_1$.  We call this the {\em underlying
    category 2-functor}. Concretely, $e_M^*\CC$ is the category
  such that $\Obj{e_M^*\CC}=\Obj{\CC}$, and a morphism from $I$ to
  $J$ is an element belonging to $\CC(I,J)(1)$, that is, $f:I\arrow_1 J$.
\item The unique monoid homomorphism $!_M:M\arrow 1$ determines the
  2-functor $!_M^*:\Cat_1\arrow\Cat_M$.  The $M$-graded category
  $!_M^*\CC$ shares the same class of objects as $\CC$, and the homset
  $!_M^*\CC(I,J)(m)$ is defined to be $\CC(I,J)$.
\end{enumerate}

There is another 2-functor $\frg M{}:\Cat_1\arrow\Cat_M$ constructing
$M$-graded categories from ordinary categories:
\begin{itemize}
\item For 0-cell $\CC\in\CATg 1$, $\frg M\CC$ is the $M$-graded category:
  \begin{align*}
  \Obj{\frg M\CC}&\triangleq \Obj{\CC},
  & \frg M\CC(I,J)(m)&\triangleq
    \begin{choice}
      \CC(I,J) & (m\ge 1) \\
      \emptyset & (\text{otherwise})
    \end{choice}
  & \up I J m n &\triangleq
                  \begin{choice}
                    \id & (m\ge 1) \\
                    ! & (\text{otherwise})
                  \end{choice}
\end{align*}
\item For 1-cell $F:\CC\arrow\DD$ in $\CATg 1$, $\frg MF:\frg M\CC\arrow \frg M\DD$
  is the $M$-graded functor:
  \begin{align*}
    (\frg MF)I\triangleq F I,\quad \frg MF_{m,I,J}(f)\triangleq
    \begin{choice}
      Ff & (m\ge 1) \\
      \id_\emptyset & (\text{otherwise})
    \end{choice}
  \end{align*}
\item For 2-cell $\alpha:F\arrow G$ in $\CATg 1$, $\frg M\alpha:\frg MF\arrow \frg MG$ is
  the $M$-graded natural transformation defined by
  $(\frg M\alpha)_I=\alpha_I$.
\end{itemize}
The verification of that the above defines a 2-functor is done by
noticing that $L$ is the {\em change-of-base} of enrichment. ***
\begin{proposition}
  There is an isomorphism of categories $\Cat_M(\frg M\CC,\DD)\cong \Cat_1(\CC,e_M^*\DD)$.
  $L$ also preserves small 2-products.
\end{proposition}
\begin{proof}
  \Th{proper proof}
  The functor $M(1,-):M\arrow\Set$ is the tensor unit of the Day's monoidal structure
  on $[M,\Set]$. Now we have $\frg M\CC(I,J)=M(1,-)\multimap\CC(I,J)=\CC(I,J)(1)$.

  $((\prod X_i)\cdot y1)(m)=(\prod X_i)\cdot M(1,m)=\prod (X_i\cdot M(1,m))$.
\end{proof}


Like binary coproducts are characterized as left adjoints to diagonal
functors, homogeneous binary coproducts has a similar
characterization. 
\begin{proposition}
  An $M$-graded category $\CC$ has homogeneous countable coproducts if
  and only if the diagonal $M$-graded functor $\CC\arrow\CC^n$ has a
  left adjoint $(+):\CC^n\arrow\CC$ in $\CAT_M$.
\end{proposition}
We can talk about functor preserving homogeneous binary
coproducts. We write $\Cat_M^+$ for the 2-category of $M$-graded
categories with homogeneous binary coproducts, $M$-graded functors
preserving homogeneous binary coproducts, and $M$-graded natural
transformations between them.

\Th{Motivating texts}

\noindent
The notion of a \emph{Freyd category} was first identified as {\em premonoidal categories} by
Robinson and Power \cite{powerrob}. Later Levy reformulated it in
terms of {\em actions} of cartesian monoidal categories.  Typically
actions are defined to be a bifunctor $\VV\times\CC\arrow\CC$
satisfying coherence axioms. In this paper, however, we would like to
consider an action of a cartesian category to an {\em $M$-graded}
category. To resolve the type mismatch, we reformulate actions as a
strong monoidal functor of type $\VV\arrow\CAT(\CC,\CC)$,
then replace $\CAT$ with the 2-category $\CAT_g$ of $M$-graded categories.

\subsection{Action of Cartesian Categories}

\begin{definition}[Categorical actions and their maps]
Let $\VV$ be a cartesian monoidal category $(\VV,1,\times)$ and
$\KK$ be a 2-category.  A {\em $\VV$-action}, denoted $(C, *)$, consists of a 0-cell $C\in\KK$
together with a strong monoidal functor
$(*):(\VV,1,\times)\arrow(\KK(C,C),\Id,\circ)$.
 A {\em map} from a
$\VV$-action $(C,*)$ to another one $(D,\star)$ is a 1-cell
$h:C\arrow D$ in $\KK$ making the following square commute:
\begin{equation}
  \label{eq:equivariant}
  \xymatrix{
    \VV \rrrh{*} \rdm{\star} & & \KK(C,C) \rdh{\KK(C,h)} \\
    \KK(D,D) \rrrm{\KK(h,D)} & & \KK(C,D)
  }
\end{equation}
\Th{We need action compatibility, like
  $h\circ (C*)\circ(D*)\cong h\circ((C\times D)*)=((C\times D)\star)\circ h$ is equal to
  $h\circ (C*)\circ(D*)=(C\star)\circ (D\star)\circ h\cong ((C\times D)\star)\circ h$
  and for unit
}
%
We write $\Act\VV\KK$ for the category of $\VV$-actions and maps
between them.
\end{definition}

Let us also check the functoriality of $\Act\VV\KK$ on
$\VV$ and $\KK$. Given a finite-product preserving functor
$F:\WW\arrow\VV$ and a 2-functor $P:\KK\arrow\LL$, a $\VV$-action
$(C,*)$ yields a $\WW$-action by composing functors:
%
\begin{align}
  \xymatrix{
    (\WW,1,\times) \rrh F & (\VV,1,\times) \rrh * & (\KK(C,C),\Id,\circ) \rrh{P_{C,C}} & (\LL(PC,PC),\Id,\circ).
  }
\end{align}
%
This extends to a functor $\Act FP:\Act\VV\KK\arrow\Act\WW\LL$. We
abbreviate $\Act FP(C,*)$ to $P\la(C,*)\ra F$. When $P$ or $F$ is the
identity (2-)functor, we drop ``$P\la$'' or ``$\ra F$''.  Of course we
have $(P\la (C,*))\ra F=P\la ((C,*)\ra F)$.

\Th{$\KK=\CAT$ case}
The standard choice of $\KK$ is $\CAT$. In this case, an action
$(\CC,*)\in\Act\VV\CAT$ consists of a functor $(*):\VV\arrow[\CC,\CC]$
together with the following natural isomorphisms satisfying certain
coherence axioms:
\begin{displaymath}
  m_{1,X}:1*X\cong X,\quad m_{I,J,X}:I*(J*X)\cong (I\times J)*X.
\end{displaymath}
Note that these arise from the lax monoidal property of $(*)$.

A map from $(\CC,*)$ to $(\DD,\star)$ is a functor $h:\CC\arrow\DD$
such that $V\star hC=h(V*C)$ holds (property~\eqref{eq:equivariant}).

\begin{lemma}
  Let $\VV$ be a cartesian category. Then the curried binary product
  functor, which we also write by $(\times):\VV\arrow\CAT(\VV,\VV)$, is
  an action of $\VV$ on $\VV$ itself. Let $\WW$ be another cartesian
  category, and $p:\VV\arrow\WW$ be a functor strictly preserving
  binary products.  Then $p$ is a map between actions of type
  $(\VV,\times)\arrow(\WW,\times)\ra p$ in $\Act\VV\CAT$.
\end{lemma}

\subsection{Graded Freyd Categories}


We are ready to define $M$-graded Freyd category.  The following
definition is designed so that it yields Freyd
categories when $M=1$.
%
\begin{definition}
  An $M$-graded Freyd category consists of a cartesian category $\VV$
  together with the following morphism in $\Act\VV{\CATg M}$:
  \begin{displaymath}
    \xymatrix{
      \frg M{}\la(\VV,\times) \rrrh I & & (\CC,*)
    }
  \end{displaymath}
  which is also identity-on-object as an $M$-graded functor.
\dnote{I don't understand this last sentence. We are saying $I$ is an
  $M$-graded functor? I guess sfrom a trivial grading category on the left?}
  A {\em map} from an $M$-graded Freyd category $I:\frg M{}\cdot(\VV,\times)\arrow (\CC,*)$
  to another one $J:\frg M{}\cdot(\WW,\times)\arrow(\DD,\star)$
  is a pair of a finite product preserving functor $p:\VV\arrow\WW$
  and a map $q:(\CC,*)\arrow (\DD,\star)\ra p$ in $\Act\VV{\CATg M}$
  making the following diagram commute:
  \begin{displaymath}
    \xymatrix{
      \frg M{}\la(\VV,\times) \rrrh{I} \rdm{L\ra p} & & (\CC,*) \rdh q \\
      \frg M{}\la(\WW,\times)\ra p \rrrm{J\ra p} & & (\DD,\star)\ra p
    }
  \end{displaymath}
  We note that the composite $q\circ I$ may not satisfy the
  identity-on-object condition, hence is not a Freyd category.  We
  write this category $\Freyd M$.
\end{definition}
We next look at how a monotone monoid homomorphism $h:N\arrow M$
induces a functor of type $\Freyd h:\Freyd M\arrow\Freyd N$.  For
this, we first introduce the natural transformation, whose component
$\alpha_{(\CC,*)}:\frg N{}\cdot (\CC,*)\arrow h^*(\frg M{}\ra
(\CC,*))$ at $(\CC,*)$ is given by
\begin{displaymath}
  \alpha_{(\CC,*)}(X)=X, \quad \alpha_{(\CC,*)}(f)=f.
\end{displaymath}
*** NEED TO CHECK THE EQUIVARIANCE ***
Then every $M$-graded Freyd category
$I:\frg M{}\ra (\VV,\times)\arrow(\CC,*)$ turns into $N$-graded one:
\begin{displaymath}
  \xymatrix{
    \frg N{}\ra(\VV,\times) \rrh{\alpha_{(\VV,\times)}}
    & h^*(\frg M{}\ra (\VV,\times)) \rrh{h^*I} & h^*(\CC,*).
  }
\end{displaymath}




We note that $L:\CATg 1\arrow\CATg M$ preserves 2-products.  Therefore
it can be restricted as a 2-functor $L^+:\CATp 1\arrow\CATp M$.
Moreover, for a distributive bi-cartesian category $\VV$, we have
$(\VV,\times)\in\Act\VV{\CATp 1}$. Hence
$L^+\la(\VV,\times)\in\Act\VV{\CATp M}$.
\begin{definition}
  An $M$-graded Freyd category with homogeneous coproducts consists of
  a distributive bi-cartesian category $(\VV,1,\times,0,+)$ with the following map in
  $\Act\VV{\CATp M}$:
  \begin{displaymath}
    \xymatrix{
      L^+\la(\VV,\times) \rrrh I & & (\CC,*)
    }
  \end{displaymath}
\end{definition}

\begin{definition}
  A graded refinement of Freyd category consists of
  \begin{itemize}
  \item A $1$-graded Freyd category
    $I:\frg 1{}\cdot(\VV,\times)\arrow (\CC,*)$,
  \item An $M$-graded Freyd category
    $\dot I:\frg M{}\cdot(\PP,\times)\arrow (\EE,\star)$,
  \item A morphism of $M$-graded Freyd categories
    $(p,q):\dot I\arrow \Freyd{!_M}(I)$ such that $p$ and $q$ are faithful.
  \end{itemize}
\end{definition}
When fully expanded, $I,\dot I,p,q$ are appropriate functors
making the following diagram in $\Act\PP{\CATg M}$ commute:
\begin{displaymath}
  \xymatrix{
    \frg M{}\la (\PP,\times) \ar[rrrr]^-{\dot I} \rdm{\frg M{}\ra p} & & & & (\EE,\star) \rdh q \\
    \frg M{}\la (\VV,\times)\ra p \rrrm{\alpha_{(\VV,\times)\ra p}}
    & & (!_M)^*\la\frg 1{}\la (\VV,\times)\ra p \rrrm{(!_M)^*\la I\ra p}
    & & (!_M)^*\la (\CC,*)\ra p
  }
\end{displaymath}
This amounts to the commutativity in $\CATg M$:
\begin{displaymath}
  \xymatrix{
    L_M\PP \rrrh{\dot I} \rdm{L_M p} & & \EE \rdh q \\
    L_M\VV \rrm{...} & (!_M)^*(L_1\VV) \rrh{(!_M)^*I} & (!_M)^*\CC
  }
\end{displaymath}


==> principles.tex <==
\dnote{Linking text that establishes where we are going with the model
  (fibration, graded cats, etc.)}  \snote{I think I wrote what I want
  to say. The contents here may be affected by further edit of the
  technical section. Therefore 60\% now.}

Central to this work is the development of a categorical framework for
Graded Hoare Logic in such a way that we can model
various impure behaviours with denotations that are refined by
predicates and grades describing this impure behaviour.
Before we unpack the details of this framework, we give
an overview of its main components.

The following diagram summarizes the relationship between the
categories at play: $\PP$ a categories of predicates, $\VV$
a category of pure computations, $\CC$ a category modelling
impure computations, and $\EE$ a `graded category' (new here) for a refined
model of computations. This diagram should not be understood as a
commutative diagram in $\CAT$ as $\EE$ is a graded category
and hence not an object of $\CAT$. The relationships are:
\begin{equation}
  \label{eq:square}
  \xymatrix{
    \PP \rdm{p} \rrrh{\dot I} & & \EE \rdh q \\
    \VV \rrrm{I} & & \CC
  }
\end{equation}
%
\begin{itemize}
\item We interpret \Lang{} using a {\em Freyd category}
  $I:\VV\arrow\CC$ with countable coproducts (also called {\em
    distributive Freyd category} \cite{STATON2014197}). This is a
  well-known categorical model of effectful computation, first
  proposed by Power and Thielecke \cite{10.1007/BFb0014560}. In this
  paper we adopt Levy's reformulation of Freyd category using
  categorical actions \cite{levy05}. The category $\VV$ models values
  and pure computations, while the category $\CC$ models effectful
  computations. They are connected by a functor $I:\VV\arrow\CC$,
  representing the inclusion of pure computations into effectful
  computations. The benefit of Freyd category is that it is less
  demanding to construct models of computational effects.  For
  instance, in a non-closed cartesian category such as the category
  $\Meas$ of measurable spaces and measurable functions, we can not
  have state monads since neither have exponential objects.  However,
  in both categories we can still have a model of first-order
  effectful computation using Freyd categories \cite{...}.

\item We interpret the basic logic introduced in Section
  \ref{sec:blogic} using a {\em coherent fibration}
  $p:\PP\arrow\VV$. The semantics is the standard one; see
  e.g. \cite{jacobscltt}.

\item We interpret the graded Hoare logic as a {\em graded Freyd
    category} $\dot I:\PP\arrow\EE$ with homogeneous coproducts (Section~\ref{sec:graded-freyd-categories}). This
  new categorical structure is designed for directly interpreting
  judgements of the graded Hoare logic\dnote{This makes it sounds bad; like we did an adhoc thing. Is this a good way to phrase it?}. \snote{This is not quite I realized - in mathematics they talk about graded categories...} The major difference from the
  ordinary Freyd category is that $\EE$ is now a {\em graded
    category}, whose hom-sets are indexed by grades.  A concise
  definition of graded categories is as categories enriched over the
  category of covariant presheaves $[M,\Set]$ over grading preordered monoid
  $M$ with Day's convolution tensor product.  However, we mainly work
  with a concrete definition of graded categories (Section~\ref{sec:graded-category}), and postpone the
  abstract description of graded categories to Section
  \ref{sec:2-cat}. A \emph{graded Freyd category} is then a graded category
  with an action of an ordinary cartesian category. The subtlety of
  defining such an action across different notions of category is also
  discussed in Section \ref{sec:2-cat}.
  \snote{If Section \ref{sec:2-cat} is omitted, we should edit this part too.}

  
\item Finally, the graded category $\EE$ has a functor $q$ into $\CC$;
  precisely this is not quite a functor because $\EE$ is a graded
  category; see Definition \ref{def:logstr} for the precise meaning.
  This functor plays the role of erasing assertions and grades of
  graded Hoare logic judgements, and extracting the denotation of
  effectful programs.
\end{itemize}
This diagram also echos the principle of {\em refinement as functors}
proposed by Melli\`es and Zeilberger \cite{DBLP:conf/popl/MelliesZ15}.
The lower part of the diagram offers an interpretation of \Lang{},
while the upper part offers a logical refinement of programs with
grading.  In short, we aim to introduce a {\em graded refinement} of
Freyd categories.


==> prodcons.tex <==
\section{Producer and Consumer Constructions}

Graded categories may be seen as categories where morphisms have
costs. From such a category, we construct an ordinary category where
each object carries an approximation of the current cost, and
morphisms {\em consume} or {\em produce} costs.

\begin{definition}
  Let $(M,\le,1,\cdot)$ be a partially ordered monoid and $\CC$ be an
  $M$-graded category. We define the {\em producer category} $P(\CC)$
  by the following data.  Objects of $P(\CC)$ are pairs $(m,I)$ where
  $m\in M$ and $I\in\CC$. Intuitively, such an object represents the
  situation where one has a value of type $I$ and the accumulated cost
  is {\em at most} $m$.  The homset from $(m,I)$ to $(n,J)$ is defined
  by the following quotient set:
  \begin{displaymath}
    P(\CC)((m,I),(n,J))=\{(p,f)~|~f\in\CC(I,J)(p),m\cdot p\le n\}/\sim
  \end{displaymath}
  where $\sim$ is the least equivalence relation such that:
  \[
    \forall p, q . \; p \le q \Rightarrow (p,f) \sim (q,\up I J p q f)
  \]
  The equivalence class of $(p,f)$ is denoted by $[p,f]$. It denotes
  computations which produce at most cost $p$ by applying $f$ and
  possibly upcasting. The cost $p$ is combined with $m$ (i.e,
  $m \cdot p$) alongside the computation of a value of type $J$, and
  yields the situation $(n,J)$.
\end{definition}

\begin{definition}
  On the other hand, the {\em consumer category} $C(\CC)$ is defined
  by the following data. Similarly to the producer category, objects
  are pairs $(m,I)$ of $m\in M$ and $I\in\CC$.  Contrary to the
  producer category, an object $(m,I)$ in the consume category
  represents that one has a value of type $I$ and the accumulated cost
  is at most $m$. The homset from $(m,I)$ to $(n,J)$ is thus defined
  by the following quotient set:
  \begin{displaymath}
    C(\CC)((m,I),(n,J))=\{(p,f)~|~f\in\CC(I,J)(p),m\ge p\cdot n\}/\sim
  \end{displaymath}
  where $\sim$ is again the same equivalence relation as above.
  % generated from $(p,f)~(q,\up I J p q f)$ for each $p\le q$. The
  % equivalence class of $(p,f)$ is denoted by $[p,f]$.
  Note that in the consumer category, morphisms $(m,I)$ to $(n,J)$ are
  those which ``consume'' costs $p$.
\end{definition}
We define the producer category $P (\EE)$ by the following data.
\begin{itemize}
\item An object is $(m, X)$ where $m \in M$ and $X \in | \EE |$. Below
  we may write $m X$ instead of $(m, X)$, and $X$ to mean $1 X$.

\item The homset is defined as follows.
  \[ P (\EE) (m X, n Y) = \{ f \in \CC (p X, p Y)~|~ \exists l \in M.m
    \cdot l \leqslant n \wedge f:X\darrow_l Y \} . \]
\end{itemize}
From this definition, we especially have
\[ P (\EE) (X, n Y) = \{ f~|~\exists l \in M.l \leqslant n \wedge
  f:X\darrow_l Y \} =\EE (X, Y) (n) . \]
\begin{proposition}
  Assume that $M$ has joins and $(\cdot)$ preserves joins. Let $\CC$
  be an $M$-graded category with homogeneous coproducts. Then the
  following holds:
  \[ f : m X \rightarrow n Z, g : m Y \rightarrow n Z \Longrightarrow
    [f, g] : m (X + Y) \rightarrow n Z. \]
\end{proposition}

\begin{proof}
  Take $p, q$ such that $m \cdot p \leqslant n$ and
  $m \cdot q \leqslant n$ and $f \in X\darrow_p Z$ and
  $g \in Y\darrow_q Z$. From the first two and the distributivity of
  $(\cdot)$ over $(\vee)$, we obtain $m \cdot (p \vee q) \leqslant
  n$. From the monotonicity, we obtain $f \in X\darrow_{p\vee q}Z$ and
  $g \in Y\darrow_{p\vee q}Z$.  Therefore
  $[f, g] \in X+Y\darrow_{p\vee q}Z$ by the homogeneous coproduct. We
  conclude $[f, g] : m (X + Y) \rightarrow n Z$ from the definition of
  $P (\EE)$ morphism.
\end{proof}

\begin{corollary}
  If $\CC$ has coproducts, and an $M$-graded refinement
  $p:\EE\arrow\CC$ has homogeneous coproducts, and $M$ has joins
  preserved by $(\cdot)$, then $p(\EE)$ has coproducts of $mX$ and
  $mY$.
\end{corollary}




% We derive two $M^{{op}}$-graded categories $M$ and $M^*$ by:
% \begin{eqnarray*}
%   M (m, m') (p) & = & M (m \cdot p, m')\\
%   M^* (m, m') (p) & = & M^* (m, p
%                         \cdot m')\\
%                 & = & M (p \cdot m', m) .
% \end{eqnarray*}
% We note that when $M$ admits inverses (i.e. $(M, 1, \cdot)$ is a
% group), we have an isomorphism $\Phi : M \rightarrow M^*$ of
% categories given by $\Phi (m) = m^{- 1}$.

% We now give a construction of an ordinary category from an
% $M$-graded category. For this, we introduce a convenient operator
% called {\em{tensor}} of presheaves. For $F : M \rightarrow \Set$ and
% $G : M^{{op}} \rightarrow \Set$, by $F \actionTensor G$ we mean the coend
% \[ F \actionTensor G = \int^{m \in M} F m \times G m. \]

% \begin{definition}
%   Let $\CC$ be an $M$-graded category. We define $P(\CC)$ (producer
%   category) by
%   \begin{itemize}
%   \item An object is a pair $(m, A)$ where $m \in M$ and
%     $A \in \CC$.

%   \item A homset is given by
%     $P (\CC) ((m, A), (n, B)) =\CC (A, B) \actionTensor M (m, n)$.
%   \end{itemize}
%   This category has $M$-action. Similarly, we define $C(\CC)$
%   (consumer category) by
%   \begin{itemize}
%   \item An object is a pair $(m, A)$ where $m \in M$ and
%     $A \in \CC$.

%   \item A homset is given by
%     $C (\CC) ((m, A), (n, B)) =\CC (A, B) \actionTensor M^* (m, n)$.
%   \end{itemize}
%   This category has an $M^{{op}}$-action.
% \end{definition}
Each of the categories $C(\CC)$ and $P(\CC)$ come with a strict
$M$-action (i.e., functors
$\-*\- : M \times C(\CC) \rightarrow C(\CC)$ and
$\-*\- : M \times P(\CC) \rightarrow P(\CC)$) defined by
$n*(m,A)=(n\cdot m,A)$. Evidently, $1*(m,A)=(m,A)$ and
$n*(n'*(m,A))=(n\cdot n')*(m,A)$ holds by monoidality of $M$.
% This is to say we have a graded monad here.

\begin{theorem}
  Let $\CC$ be an $M$-graded category. Then it is the full subcategory
  of the Kleisli $M$-graded category of the strict action $(*)$,
  (State this as a form of adjunction)
\end{theorem}
\begin{proof}
  From the co-Yoneda lemma we obtain:
  \begin{align*}
    P (\CC) ((1, A), m*(1, B)) & = \int^p \CC (A, B) (p) \times M (p, m)\\
                               & \cong \CC (A, B) (m).
  \end{align*}
  \dnote{Relate to the construction in~\cite{fujii2016towards}.}
\end{proof}
This construction, together with the on $P(\CC_T)$
% Dually
% \[ C (\CC) ((m, A), (1, B)) = \int^p \CC (A, B) (p) \times M^* (p,
%   m) \cong \CC (A, B) (m) . \]

% \dnote{This gives a link back to
% Section~\ref{subsec:graded-cat-to-graded-monads-and-comonads}
% perhaps we ought to combine them? I think this would make sense and
% we can tell a more coherent story about linking the product/consume
% to graded monads/comonads.}

% \begin{theorem}
%   Assume that $M$ is commutative. For any $M$-graded symmetric
%   monoidal category $\CC$, ${Kl} (\CC)$ also has the symmetric
%   monoidal structure given by
%   \[ (m A) \otimes (n B) = (m \cdot n, A \otimes B) . \]
% \end{theorem}

% Conjecture: Suppose that $M$ admits joins and $(\cdot)$ preserves
% joins in each argument. Then for any $M$-graded category $\CC$
% admitting homogeneous coproduct, $Kl (\CC)$ admits coproducts of
% $m A$ and $m B$.


\Th{The following is producer/consumer construction examples}

\begin{example}

Now we calculate $\mathrm{Kl}(\Pred_{\mathcal{U}})$.
\begin{itemize}
\item An objects is a pair $(\delta,(X,P))$ where
  $\delta \in \mathbb{R}_{\geq 0}$ and $(X,P)\in\Pred$
\item
  $\mathrm{Kl}(\Pred_{\mathcal{U}})((\delta_1,(X,P)),(\delta_2,(Y,Q)))
  = \Pred_{\mathcal{U}}((X,P),(Y,Q)) \actionTensor{} \mathbb{R}_{\geq 0}(\delta,
  \delta')$.
\end{itemize}
At all we have,
\begin{align*}
  \lefteqn{
  \Pred_{\mathcal{U}}((X,P),(Y,Q)) \actionTensor{} \mathbb{R}_{\geq 0}(\delta_1, \delta_2)}
  \\
& \cong
  \set{
  f \colon X \to Y \in \Set_{\mathcal{D}}
  \mid
  \begin{array}{l}
    \exists
    \delta' \in \mathbb{R}_{\geq 0} \text{ s.t. } \\
    \delta_1 + \delta' \leq \delta_2.~
    f \colon (X,P) \dto \mathcal{U}^{\delta'}(Y,Q)
  \end{array}
  }
\end{align*}
We also calculate $\mathrm{coKl}(\Pred_{\mathcal{U}})$.  For Hom-sets,
in the similar way as above, we obtain
\begin{align*}
  \lefteqn{
  \mathrm{coKl}(\Pred_{\mathcal{U}})((\delta_1,(X,P)),(\delta_2,(Y,Q)))
  }
  \\
&
  =
  \Pred_{\mathcal{U}}((X,P),(Y,Q)) \actionTensor{} \mathbb{R}_{\geq 0}^{\mathrm{op}}(\delta_1, \delta_2)
  \\
& \cong
  \set{
  f \colon X \to Y \in \Set_{\mathcal{D}}
  \mid
  \begin{array}{l}
    \exists
    \delta' \in \mathbb{R}_{\geq 0} \text{ s.t. }\\
    \delta_1 \geq \delta' + \delta_2.~
    f \colon (X,P) \dto \mathcal{U}^{\delta'}(Y,Q)
  \end{array}
  }
\end{align*}
\end{example}

